Syntheto: A Surface Language for APT and ACL2

Syntheto is a surface language for carrying out formally verified program synthesis by transformational refinement in ACL2 using the APT toolkit. Syntheto aims at providing more familiarity and automation, in order to make this technology more widely usable. Syntheto is a strongly statically typed functional language that includes both executable and non-executable constructs, including facilities to state and prove theorems and facilities to apply proof-generating transformations. Syntheto is integrated into an IDE with a notebook-style, interactive interface that translates Syntheto to ACL2 definitions and APT transformation invocations, and back-translates the prover's results to Syntheto; the bidirectional translation happens behind the scenes, with the user interacting solely with Syntheto.

==> eptcsdata.tex <==
\providecommand{\firstpage}{151}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.13}{10.4204/EPTCS.359.13}}
\pdfoutput=1

